Optical Identification and Spectroscopy of Supernova Remnants in the Galaxy M51

Using a combination of ground-based and HST imaging, we have constructed a catalog of 179 supernova remnants (SNRs) and SNR candidates in the nearby spiral galaxy M51. Follow-up spectroscopy of 66 of the candidates confirms 61 of these as SNRs, and suggests that the vast majority of the unobserved objects are SNRs as well. A total of 55 of the candidates are coincident with (mostly soft) X-ray sources identified in deep Chandra observations of M51; searching the positions of other soft X-ray sources resulted in several additional possible optical candidates. There are 16 objects in the catalog coincident with known radio sources. None of the sources with spectra shows the high velocities (>500 km/s) characteristic of young, ejecta-dominated SNRs like Cas A; instead, most if not all appear to be middle-aged SNRs. The general properties of the SNRs, size distribution and spectral characteristics, resemble those in other nearby spiral galaxies, notably M33, M83, and NGC6946, where similar samples exist. However, the spectroscopically observed [N II]:H{\alpha} ratios appear to be significantly higher than in any of these other galaxies. Although we have explored various ideas to explain the high ratios in M51, none of the explanations appears to be satisfactory.

==> table5_obs_spect.tex <==
%  SN1006 core sample paper,  Table 1
\begin{deluxetable}{ccccc}
%\rotate
%\tablewidth{600pt}
\tablewidth{0pt}
%\tabletypesize{small}
\tablecaption{Gemini-N/GMOS Multi-Object Spectroscopy Observations of M51 \label{table5_obs_spectra}}

\tablehead{
\colhead{Mask No.} &
\multicolumn{2}{c}{Center Position} &
\colhead{Date (UT)}  &
%\colhead{CWLs} &
\colhead{Total Exposure (s)\tablenotemark{a} }\\
\colhead{} & \multicolumn{2}{c}{R.A.\phn\,(J2000.)\, Decl.} & \colhead{} & \colhead{}
%\colhead{Comments} 
%\colhead{$\rm \lambda_{c}[corr]$(\AA)\tablenotemark{b}} &
%\colhead{$\Delta \lambda$(\AA)\tablenotemark{a}} &
%\colhead {Exposure (s)} 
}
%\tabletypesize{\normal}
\tablewidth{0pt}
\startdata
%2 & 7 Apr 2011 & $7 \times 1000$ &  Variable clouds and seeing  \\[-8pt]
% &  & $7 \times 1000$ &    \\[-9pt]
 %& 7 Apr 2011 &  &  Variable clouds and seeing  \\[-9pt]
%2 &    &  $2 \times 1500$ &  \\[-1pt]
%&  9 Apr 2011  & $2 \times 1400$ & Clear; seeing $<1\arcsec$  \\[2pt]
%% & 9 Apr 2011 & $ 1500 + 1350 $ &  Clear; seeing $\lesssim 0\farcs 7$  \\
 1 & 13:29:57.4\phn\phn & \phn\phn47:11:40 & 2018 May 7-8 & 3 CWLs\,$\times 4 \times 1100$  \\[2pt]
 2 & 13:29:49.0\phn\phn & \phn\phn47:11:15   & 2018 May 12 & 3 CWLs\,$\times 4 \times 1100$ \\[2pt]
 & & & & 2 CWLs\,$\times 4 \times 1100$ \\[-7.5pt]
3 & 13:29:57.4\phn\phn & \phn\phn47:11:40  & 2018 Jun 7\,-\,Jul 14 &   \\[-7.5pt]
 & & & & 1 CWL\phn $\times 2 \times 1100$ \\[2pt]
\enddata

\tablenotetext{a}{Number of different Central Wavelength Settings $\times$ number of exposures at each CWL $\times$ individual exposure time.}

\end{deluxetable}



